Higher Order Continuity for Smooth As-Rigid-As-Possible Shape Modeling

We propose a modification of the As-Rigid-As-Possible (ARAP) mesh deformation energy with higher order smoothness, which overcomes a prominent limitation of the original ARAP formulation: spikes and lack of continuity at the manipulation handles. Our method avoids spikes even when using single-point positional constraints. Since no explicit rotations have to be specified, the user interaction can be realized through a simple click-and-drag interface, where points on the mesh can be selected and moved around while the rest of the mesh surface automatically deforms accordingly. Our method preserves the benefits of ARAP deformations: it is easy to implement and thus useful for practical applications, while its efficiency makes it usable in real-time, interactive scenarios on detailed models.

==> figures/tikz_plot/edge_only.tex <==
\addplot [color=mycolor2, solid, line width=1.3pt]
table[row sep=crcr]{%
1 0.00133947\\
2 0.000834961\\
3 0.000706877\\
4 0.000676223\\
5 0.00066913\\
6 0.000667658\\
7 0.000667468\\
8 0.000667526\\
9 0.000667602\\
10 0.000667655\\
11 0.000667688\\
12 0.000667707\\
13 0.000667717\\
14 0.000667722\\
15 0.000667725\\
16 0.000667726\\
17 0.000667726\\
18 0.000667726\\
19 0.000667725\\
20 0.000667725\\
21 0.000667725\\
22 0.000667724\\
23 0.000667724\\
24 0.000667724\\
25 0.000667724\\
26 0.000667724\\
27 0.000667724\\
28 0.000667724\\
29 0.000667724\\
30 0.000667724\\
31 0.000667723\\
32 0.000667723\\
33 0.000667723\\
34 0.000667723\\
35 0.000667723\\
36 0.000667723\\
37 0.000667723\\
38 0.000667723\\
39 0.000667723\\
40 0.000667723\\
41 0.000667723\\
42 0.000667723\\
43 0.000667723\\
44 0.000667723\\
45 0.000667723\\
46 0.000667723\\
47 0.000667723\\
48 0.000667723\\
49 0.000667723\\
50 0.000667723\\
51 0.000667723\\
52 0.000667723\\
53 0.000667723\\
54 0.000667723\\
55 0.000667723\\
56 0.000667723\\
57 0.000667723\\
58 0.000667723\\
59 0.000667723\\
60 0.000667723\\
61 0.000667723\\
62 0.000667723\\
63 0.000667723\\
64 0.000667723\\
65 0.000667723\\
66 0.000667723\\
67 0.000667723\\
68 0.000667723\\
69 0.000667723\\
70 0.000667723\\
71 0.000667723\\
72 0.000667723\\
73 0.000667723\\
74 0.000667723\\
75 0.000667723\\
76 0.000667723\\
77 0.000667723\\
78 0.000667723\\
79 0.000667723\\
80 0.000667723\\
81 0.000667723\\
82 0.000667723\\
83 0.000667723\\
84 0.000667723\\
85 0.000667723\\
86 0.000667723\\
87 0.000667723\\
88 0.000667723\\
89 0.000667723\\
90 0.000667723\\
91 0.000667723\\
92 0.000667723\\
93 0.000667723\\
94 0.000667723\\
95 0.000667723\\
96 0.000667723\\
97 0.000667723\\
98 0.000667723\\
99 0.000667723\\
100 0.000667723\\
101 0.000667723\\
102 0.000667723\\
103 0.000667723\\
104 0.000667723\\
105 0.000667723\\
106 0.000667723\\
107 0.000667723\\
108 0.000667723\\
109 0.000667723\\
110 0.000667723\\
111 0.000667723\\
112 0.000667723\\
113 0.000667723\\
114 0.000667723\\
115 0.000667723\\
116 0.000667723\\
117 0.000667723\\
118 0.000667723\\
119 0.000667723\\
120 0.000667723\\
121 0.000667723\\
122 0.000667723\\
123 0.000667723\\
124 0.000667723\\
125 0.000667723\\
126 0.000667723\\
127 0.000667723\\
128 0.000667723\\
129 0.000667723\\
130 0.000667723\\
131 0.000667723\\
132 0.000667723\\
133 0.000667723\\
134 0.000667723\\
135 0.000667723\\
136 0.000667723\\
137 0.000667723\\
138 0.000667723\\
139 0.000667723\\
140 0.000667723\\
141 0.000667723\\
142 0.000667723\\
143 0.000667723\\
144 0.000667723\\
145 0.000667723\\
146 0.000667723\\
147 0.000667723\\
148 0.000667723\\
149 0.000667723\\
150 0.000667723\\
151 0.000667723\\
152 0.000667723\\
153 0.000667723\\
154 0.000667723\\
155 0.000667723\\
156 0.000667723\\
157 0.000667723\\
158 0.000667723\\
159 0.000667723\\
160 0.000667723\\
161 0.000667723\\
162 0.000667723\\
163 0.000667723\\
164 0.000667723\\
165 0.000667723\\
166 0.000667723\\
167 0.000667723\\
168 0.000667723\\
169 0.000667723\\
170 0.000667723\\
171 0.000667723\\
172 0.000667723\\
173 0.000667723\\
174 0.000667723\\
175 0.000667723\\
176 0.000667723\\
177 0.000667723\\
178 0.000667723\\
179 0.000667723\\
180 0.000667723\\
181 0.000667723\\
182 0.000667723\\
183 0.000667723\\
184 0.000667723\\
185 0.000667723\\
186 0.000667723\\
187 0.000667723\\
188 0.000667723\\
189 0.000667723\\
190 0.000667723\\
191 0.000667723\\
192 0.000667723\\
193 0.000667723\\
194 0.000667723\\
195 0.000667723\\
196 0.000667723\\
197 0.000667723\\
198 0.000667723\\
199 0.000667723\\
200 0.000667723\\
201 0.000667723\\
202 0.000667723\\
203 0.000667723\\
204 0.000667723\\
205 0.000667723\\
206 0.000667723\\
207 0.000667723\\
208 0.000667723\\
209 0.000667723\\
210 0.000667723\\
211 0.000667723\\
212 0.000667723\\
213 0.000667723\\
214 0.000667723\\
215 0.000667723\\
216 0.000667723\\
217 0.000667723\\
218 0.000667723\\
219 0.000667723\\
220 0.000667723\\
221 0.000667723\\
222 0.000667723\\
223 0.000667723\\
224 0.000667723\\
225 0.000667723\\
226 0.000667723\\
227 0.000667723\\
228 0.000667723\\
229 0.000667723\\
230 0.000667723\\
231 0.000667723\\
232 0.000667723\\
233 0.000667723\\
234 0.000667723\\
235 0.000667723\\
236 0.000667723\\
237 0.000667723\\
238 0.000667723\\
239 0.000667723\\
240 0.000667723\\
241 0.000667723\\
242 0.000667723\\
243 0.000667723\\
244 0.000667723\\
245 0.000667723\\
246 0.000667723\\
247 0.000667723\\
248 0.000667723\\
249 0.000667723\\
250 0.000667723\\
251 0.000667723\\
252 0.000667723\\
253 0.000667723\\
254 0.000667723\\
255 0.000667723\\
256 0.000667723\\
257 0.000667723\\
258 0.000667723\\
259 0.000667723\\
260 0.000667723\\
261 0.000667723\\
262 0.000667723\\
263 0.000667723\\
264 0.000667723\\
265 0.000667723\\
266 0.000667723\\
267 0.000667723\\
268 0.000667723\\
269 0.000667723\\
270 0.000667723\\
271 0.000667723\\
272 0.000667723\\
273 0.000667723\\
274 0.000667723\\
275 0.000667723\\
276 0.000667723\\
277 0.000667723\\
278 0.000667723\\
279 0.000667723\\
280 0.000667723\\
281 0.000667723\\
282 0.000667723\\
283 0.000667723\\
284 0.000667723\\
285 0.000667723\\
286 0.000667723\\
287 0.000667723\\
288 0.000667723\\
289 0.000667723\\
290 0.000667723\\
291 0.000667723\\
292 0.000667723\\
293 0.000667723\\
294 0.000667723\\
295 0.000667723\\
296 0.000667723\\
297 0.000667723\\
298 0.000667723\\
299 0.000667723\\
300 0.000667723\\
301 0.000667723\\
302 0.000667723\\
303 0.000667723\\
304 0.000667723\\
305 0.000667723\\
306 0.000667723\\
307 0.000667723\\
308 0.000667723\\
309 0.000667723\\
310 0.000667723\\
311 0.000667723\\
312 0.000667723\\
313 0.000667723\\
314 0.000667723\\
315 0.000667723\\
316 0.000667723\\
317 0.000667723\\
318 0.000667723\\
319 0.000667723\\
320 0.000667723\\
321 0.000667723\\
322 0.000667723\\
323 0.000667723\\
324 0.000667723\\
325 0.000667723\\
326 0.000667723\\
327 0.000667723\\
328 0.000667723\\
329 0.000667723\\
330 0.000667723\\
331 0.000667723\\
332 0.000667723\\
333 0.000667723\\
334 0.000667723\\
335 0.000667723\\
336 0.000667723\\
337 0.000667723\\
338 0.000667723\\
339 0.000667723\\
340 0.000667723\\
341 0.000667723\\
342 0.000667723\\
343 0.000667723\\
344 0.000667723\\
345 0.000667723\\
346 0.000667723\\
347 0.000667723\\
348 0.000667723\\
349 0.000667723\\
350 0.000667723\\
351 0.000667723\\
352 0.000667723\\
353 0.000667723\\
354 0.000667723\\
355 0.000667723\\
356 0.000667723\\
357 0.000667723\\
358 0.000667723\\
359 0.000667723\\
360 0.000667723\\
361 0.000667723\\
362 0.000667723\\
363 0.000667723\\
364 0.000667723\\
365 0.000667723\\
366 0.000667723\\
367 0.000667723\\
368 0.000667723\\
369 0.000667723\\
370 0.000667723\\
371 0.000667723\\
372 0.000667723\\
373 0.000667723\\
374 0.000667723\\
375 0.000667723\\
376 0.000667723\\
377 0.000667723\\
378 0.000667723\\
379 0.000667723\\
380 0.000667723\\
381 0.000667723\\
382 0.000667723\\
383 0.000667723\\
384 0.000667723\\
385 0.000667723\\
386 0.000667723\\
387 0.000667723\\
388 0.000667723\\
389 0.000667723\\
390 0.000667723\\
391 0.000667723\\
392 0.000667723\\
393 0.000667723\\
394 0.000667723\\
395 0.000667723\\
396 0.000667723\\
397 0.000667723\\
398 0.000667723\\
399 0.000667723\\
400 0.000667723\\
401 0.000667723\\
402 0.000667723\\
403 0.000667723\\
404 0.000667723\\
405 0.000667723\\
406 0.000667723\\
407 0.000667723\\
408 0.000667723\\
409 0.000667723\\
410 0.000667723\\
411 0.000667723\\
412 0.000667723\\
413 0.000667723\\
414 0.000667723\\
415 0.000667723\\
416 0.000667723\\
417 0.000667723\\
418 0.000667723\\
419 0.000667723\\
420 0.000667723\\
421 0.000667723\\
422 0.000667723\\
423 0.000667723\\
424 0.000667723\\
425 0.000667723\\
426 0.000667723\\
427 0.000667723\\
428 0.000667723\\
429 0.000667723\\
430 0.000667723\\
431 0.000667723\\
432 0.000667723\\
433 0.000667723\\
434 0.000667723\\
435 0.000667723\\
436 0.000667723\\
437 0.000667723\\
438 0.000667723\\
439 0.000667723\\
440 0.000667723\\
441 0.000667723\\
442 0.000667723\\
443 0.000667723\\
444 0.000667723\\
445 0.000667723\\
446 0.000667723\\
447 0.000667723\\
448 0.000667723\\
449 0.000667723\\
450 0.000667723\\
451 0.000667723\\
452 0.000667723\\
453 0.000667723\\
454 0.000667723\\
455 0.000667723\\
456 0.000667723\\
457 0.000667723\\
458 0.000667723\\
459 0.000667723\\
460 0.000667723\\
461 0.000667723\\
462 0.000667723\\
463 0.000667723\\
464 0.000667723\\
465 0.000667723\\
466 0.000667723\\
467 0.000667723\\
468 0.000667723\\
469 0.000667723\\
470 0.000667723\\
471 0.000667723\\
472 0.000667723\\
473 0.000667723\\
474 0.000667723\\
475 0.000667723\\
476 0.000667723\\
477 0.000667723\\
478 0.000667723\\
479 0.000667723\\
480 0.000667723\\
481 0.000667723\\
482 0.000667723\\
483 0.000667723\\
484 0.000667723\\
485 0.000667723\\
486 0.000667723\\
487 0.000667723\\
488 0.000667723\\
489 0.000667723\\
490 0.000667723\\
491 0.000667723\\
492 0.000667723\\
493 0.000667723\\
494 0.000667723\\
495 0.000667723\\
496 0.000667723\\
497 0.000667723\\
498 0.000667723\\
499 0.000667723\\
500 0.000667723\\
501 0.000667723\\
502 0.000667723\\
503 0.000667723\\
504 0.000667723\\
505 0.000667723\\
506 0.000667723\\
507 0.000667723\\
508 0.000667723\\
509 0.000667723\\
510 0.000667723\\
511 0.000667723\\
512 0.000667723\\
513 0.000667723\\
514 0.000667723\\
515 0.000667723\\
516 0.000667723\\
517 0.000667723\\
518 0.000667723\\
519 0.000667723\\
520 0.000667723\\
521 0.000667723\\
522 0.000667723\\
523 0.000667723\\
524 0.000667723\\
525 0.000667723\\
526 0.000667723\\
527 0.000667723\\
528 0.000667723\\
529 0.000667723\\
530 0.000667723\\
531 0.000667723\\
532 0.000667723\\
533 0.000667723\\
534 0.000667723\\
535 0.000667723\\
536 0.000667723\\
537 0.000667723\\
538 0.000667723\\
539 0.000667723\\
540 0.000667723\\
541 0.000667723\\
542 0.000667723\\
543 0.000667723\\
544 0.000667723\\
545 0.000667723\\
546 0.000667723\\
547 0.000667723\\
548 0.000667723\\
549 0.000667723\\
550 0.000667723\\
551 0.000667723\\
552 0.000667723\\
553 0.000667723\\
554 0.000667723\\
555 0.000667723\\
556 0.000667723\\
557 0.000667723\\
558 0.000667723\\
559 0.000667723\\
560 0.000667723\\
561 0.000667723\\
562 0.000667723\\
563 0.000667723\\
564 0.000667723\\
565 0.000667723\\
566 0.000667723\\
567 0.000667723\\
568 0.000667723\\
569 0.000667723\\
570 0.000667723\\
571 0.000667723\\
572 0.000667723\\
573 0.000667723\\
574 0.000667723\\
575 0.000667723\\
576 0.000667723\\
577 0.000667723\\
578 0.000667723\\
579 0.000667723\\
580 0.000667723\\
581 0.000667723\\
582 0.000667723\\
583 0.000667723\\
584 0.000667723\\
585 0.000667723\\
586 0.000667723\\
587 0.000667723\\
588 0.000667723\\
589 0.000667723\\
590 0.000667723\\
591 0.000667723\\
592 0.000667723\\
593 0.000667723\\
594 0.000667723\\
595 0.000667723\\
596 0.000667723\\
597 0.000667723\\
598 0.000667723\\
599 0.000667723\\
600 0.000667723\\
601 0.000667723\\
602 0.000667723\\
603 0.000667723\\
604 0.000667723\\
605 0.000667723\\
606 0.000667723\\
607 0.000667723\\
608 0.000667723\\
609 0.000667723\\
610 0.000667723\\
611 0.000667723\\
612 0.000667723\\
613 0.000667723\\
614 0.000667723\\
615 0.000667723\\
616 0.000667723\\
617 0.000667723\\
618 0.000667723\\
619 0.000667723\\
620 0.000667723\\
621 0.000667723\\
622 0.000667723\\
623 0.000667723\\
624 0.000667723\\
625 0.000667723\\
626 0.000667723\\
627 0.000667723\\
628 0.000667723\\
629 0.000667723\\
630 0.000667723\\
631 0.000667723\\
632 0.000667723\\
633 0.000667723\\
634 0.000667723\\
635 0.000667723\\
636 0.000667723\\
637 0.000667723\\
638 0.000667723\\
639 0.000667723\\
640 0.000667723\\
641 0.000667723\\
642 0.000667723\\
643 0.000667723\\
644 0.000667723\\
645 0.000667723\\
646 0.000667723\\
647 0.000667723\\
648 0.000667723\\
649 0.000667723\\
650 0.000667723\\
651 0.000667723\\
652 0.000667723\\
653 0.000667723\\
654 0.000667723\\
655 0.000667723\\
656 0.000667723\\
657 0.000667723\\
658 0.000667723\\
659 0.000667723\\
660 0.000667723\\
661 0.000667723\\
662 0.000667723\\
663 0.000667723\\
664 0.000667723\\
665 0.000667723\\
666 0.000667723\\
667 0.000667723\\
668 0.000667723\\
669 0.000667723\\
670 0.000667723\\
671 0.000667723\\
672 0.000667723\\
673 0.000667723\\
674 0.000667723\\
675 0.000667723\\
676 0.000667723\\
677 0.000667723\\
678 0.000667723\\
679 0.000667723\\
680 0.000667723\\
681 0.000667723\\
682 0.000667723\\
683 0.000667723\\
684 0.000667723\\
685 0.000667723\\
686 0.000667723\\
687 0.000667723\\
688 0.000667723\\
689 0.000667723\\
690 0.000667723\\
691 0.000667723\\
692 0.000667723\\
693 0.000667723\\
694 0.000667723\\
695 0.000667723\\
696 0.000667723\\
697 0.000667723\\
698 0.000667723\\
699 0.000667723\\
700 0.000667723\\
701 0.000667723\\
702 0.000667723\\
703 0.000667723\\
704 0.000667723\\
705 0.000667723\\
706 0.000667723\\
707 0.000667723\\
708 0.000667723\\
709 0.000667723\\
710 0.000667723\\
711 0.000667723\\
712 0.000667723\\
713 0.000667723\\
714 0.000667723\\
715 0.000667723\\
716 0.000667723\\
717 0.000667723\\
718 0.000667723\\
719 0.000667723\\
720 0.000667723\\
721 0.000667723\\
722 0.000667723\\
723 0.000667723\\
724 0.000667723\\
725 0.000667723\\
726 0.000667723\\
727 0.000667723\\
728 0.000667723\\
729 0.000667723\\
730 0.000667723\\
731 0.000667723\\
732 0.000667723\\
733 0.000667723\\
734 0.000667723\\
735 0.000667723\\
736 0.000667723\\
737 0.000667723\\
738 0.000667723\\
739 0.000667723\\
740 0.000667723\\
741 0.000667723\\
742 0.000667723\\
743 0.000667723\\
744 0.000667723\\
745 0.000667723\\
746 0.000667723\\
747 0.000667723\\
748 0.000667723\\
749 0.000667723\\
750 0.000667723\\
751 0.000667723\\
752 0.000667723\\
753 0.000667723\\
754 0.000667723\\
755 0.000667723\\
756 0.000667723\\
757 0.000667723\\
758 0.000667723\\
759 0.000667723\\
760 0.000667723\\
761 0.000667723\\
762 0.000667723\\
763 0.000667723\\
764 0.000667723\\
765 0.000667723\\
766 0.000667723\\
767 0.000667723\\
768 0.000667723\\
769 0.000667723\\
770 0.000667723\\
771 0.000667723\\
772 0.000667723\\
773 0.000667723\\
774 0.000667723\\
775 0.000667723\\
776 0.000667723\\
777 0.000667723\\
778 0.000667723\\
779 0.000667723\\
780 0.000667723\\
781 0.000667723\\
782 0.000667723\\
783 0.000667723\\
784 0.000667723\\
785 0.000667723\\
786 0.000667723\\
787 0.000667723\\
788 0.000667723\\
789 0.000667723\\
790 0.000667723\\
791 0.000667723\\
792 0.000667723\\
793 0.000667723\\
794 0.000667723\\
795 0.000667723\\
796 0.000667723\\
797 0.000667723\\
798 0.000667723\\
799 0.000667723\\
800 0.000667723\\
801 0.000667723\\
802 0.000667723\\
803 0.000667723\\
804 0.000667723\\
805 0.000667723\\
806 0.000667723\\
807 0.000667723\\
808 0.000667723\\
809 0.000667723\\
810 0.000667723\\
811 0.000667723\\
812 0.000667723\\
813 0.000667723\\
814 0.000667723\\
815 0.000667723\\
816 0.000667723\\
817 0.000667723\\
818 0.000667723\\
819 0.000667723\\
820 0.000667723\\
821 0.000667723\\
822 0.000667723\\
823 0.000667723\\
824 0.000667723\\
825 0.000667723\\
826 0.000667723\\
827 0.000667723\\
828 0.000667723\\
829 0.000667723\\
830 0.000667723\\
831 0.000667723\\
832 0.000667723\\
833 0.000667723\\
834 0.000667723\\
835 0.000667723\\
836 0.000667723\\
837 0.000667723\\
838 0.000667723\\
839 0.000667723\\
840 0.000667723\\
841 0.000667723\\
842 0.000667723\\
843 0.000667723\\
844 0.000667723\\
845 0.000667723\\
846 0.000667723\\
847 0.000667723\\
848 0.000667723\\
849 0.000667723\\
850 0.000667723\\
851 0.000667723\\
852 0.000667723\\
853 0.000667723\\
854 0.000667723\\
855 0.000667723\\
856 0.000667723\\
857 0.000667723\\
858 0.000667723\\
859 0.000667723\\
860 0.000667723\\
861 0.000667723\\
862 0.000667723\\
863 0.000667723\\
864 0.000667723\\
865 0.000667723\\
866 0.000667723\\
867 0.000667723\\
868 0.000667723\\
869 0.000667723\\
870 0.000667723\\
871 0.000667723\\
872 0.000667723\\
873 0.000667723\\
874 0.000667723\\
875 0.000667723\\
876 0.000667723\\
877 0.000667723\\
878 0.000667723\\
879 0.000667723\\
880 0.000667723\\
881 0.000667723\\
882 0.000667723\\
883 0.000667723\\
884 0.000667723\\
885 0.000667723\\
886 0.000667723\\
887 0.000667723\\
888 0.000667723\\
889 0.000667723\\
890 0.000667723\\
891 0.000667723\\
892 0.000667723\\
893 0.000667723\\
894 0.000667723\\
895 0.000667723\\
896 0.000667723\\
897 0.000667723\\
898 0.000667723\\
899 0.000667723\\
900 0.000667723\\
901 0.000667723\\
902 0.000667723\\
903 0.000667723\\
904 0.000667723\\
905 0.000667723\\
906 0.000667723\\
907 0.000667723\\
908 0.000667723\\
909 0.000667723\\
910 0.000667723\\
911 0.000667723\\
912 0.000667723\\
913 0.000667723\\
914 0.000667723\\
915 0.000667723\\
916 0.000667723\\
917 0.000667723\\
918 0.000667723\\
919 0.000667723\\
920 0.000667723\\
921 0.000667723\\
922 0.000667723\\
923 0.000667723\\
924 0.000667723\\
925 0.000667723\\
926 0.000667723\\
927 0.000667723\\
928 0.000667723\\
929 0.000667723\\
930 0.000667723\\
931 0.000667723\\
932 0.000667723\\
933 0.000667723\\
934 0.000667723\\
935 0.000667723\\
936 0.000667723\\
937 0.000667723\\
938 0.000667723\\
939 0.000667723\\
940 0.000667723\\
941 0.000667723\\
942 0.000667723\\
943 0.000667723\\
944 0.000667723\\
945 0.000667723\\
946 0.000667723\\
947 0.000667723\\
948 0.000667723\\
949 0.000667723\\
950 0.000667723\\
951 0.000667723\\
952 0.000667723\\
953 0.000667723\\
954 0.000667723\\
955 0.000667723\\
956 0.000667723\\
957 0.000667723\\
958 0.000667723\\
959 0.000667723\\
960 0.000667723\\
961 0.000667723\\
962 0.000667723\\
963 0.000667723\\
964 0.000667723\\
965 0.000667723\\
966 0.000667723\\
967 0.000667723\\
968 0.000667723\\
969 0.000667723\\
970 0.000667723\\
971 0.000667723\\
972 0.000667723\\
973 0.000667723\\
974 0.000667723\\
975 0.000667723\\
976 0.000667723\\
977 0.000667723\\
978 0.000667723\\
979 0.000667723\\
980 0.000667723\\
981 0.000667723\\
982 0.000667723\\
983 0.000667723\\
984 0.000667723\\
985 0.000667723\\
986 0.000667723\\
987 0.000667723\\
988 0.000667723\\
989 0.000667723\\
990 0.000667723\\
991 0.000667723\\
992 0.000667723\\
993 0.000667723\\
994 0.000667723\\
995 0.000667723\\
996 0.000667723\\
997 0.000667723\\
998 0.000667723\\
999 0.000667723\\
1000 0.000667723\\
};
\addlegendentry{edge-only}

==> figures/tikz_plot/full.tex <==
\addplot [color=mycolor1, solid, line width=1.3pt]
table[row sep=crcr]{%
1 0.00133947\\
2 0.00131433\\
3 0.00132216\\
4 0.00132919\\
5 0.00133421\\
6 0.00133741\\
7 0.00133908\\
8 0.00133947\\
9 0.00133881\\
10 0.00133731\\
11 0.00133513\\
12 0.00133241\\
13 0.00132926\\
14 0.00132578\\
15 0.00132204\\
16 0.00131809\\
17 0.001314\\
18 0.00130978\\
19 0.00130548\\
20 0.00130111\\
21 0.00129669\\
22 0.00129224\\
23 0.00128777\\
24 0.00128328\\
25 0.00127881\\
26 0.00127434\\
27 0.0012699\\
28 0.00126549\\
29 0.00126112\\
30 0.0012568\\
31 0.00125254\\
32 0.00124834\\
33 0.00124422\\
34 0.00124017\\
35 0.00123621\\
36 0.00123235\\
37 0.00122857\\
38 0.00122489\\
39 0.00122132\\
40 0.00121785\\
41 0.00121449\\
42 0.00121123\\
43 0.00120809\\
44 0.00120506\\
45 0.00120214\\
46 0.00119933\\
47 0.00119664\\
48 0.00119406\\
49 0.0011916\\
50 0.00118924\\
51 0.001187\\
52 0.00118487\\
53 0.00118286\\
54 0.00118095\\
55 0.00117914\\
56 0.00117745\\
57 0.00117586\\
58 0.00117438\\
59 0.001173\\
60 0.00117172\\
61 0.00117054\\
62 0.00116946\\
63 0.00116847\\
64 0.00116759\\
65 0.00116679\\
66 0.00116609\\
67 0.00116547\\
68 0.00116495\\
69 0.00116451\\
70 0.00116416\\
71 0.00116389\\
72 0.0011637\\
73 0.00116359\\
74 0.00116356\\
75 0.00116361\\
76 0.00116373\\
77 0.00116393\\
78 0.0011642\\
79 0.00116453\\
80 0.00116494\\
81 0.00116541\\
82 0.00116595\\
83 0.00116655\\
84 0.00116721\\
85 0.00116794\\
86 0.00116872\\
87 0.00116956\\
88 0.00117045\\
89 0.0011714\\
90 0.0011724\\
91 0.00117346\\
92 0.00117456\\
93 0.00117571\\
94 0.00117691\\
95 0.00117816\\
96 0.00117945\\
97 0.00118078\\
98 0.00118215\\
99 0.00118357\\
100 0.00118502\\
101 0.00118651\\
102 0.00118804\\
103 0.0011896\\
104 0.0011912\\
105 0.00119283\\
106 0.00119449\\
107 0.00119619\\
108 0.00119791\\
109 0.00119966\\
110 0.00120144\\
111 0.00120325\\
112 0.00120508\\
113 0.00120693\\
114 0.00120881\\
115 0.00121071\\
116 0.00121263\\
117 0.00121457\\
118 0.00121653\\
119 0.00121851\\
120 0.00122051\\
121 0.00122252\\
122 0.00122455\\
123 0.0012266\\
124 0.00122866\\
125 0.00123073\\
126 0.00123282\\
127 0.00123491\\
128 0.00123702\\
129 0.00123914\\
130 0.00124126\\
131 0.0012434\\
132 0.00124554\\
133 0.0012477\\
134 0.00124985\\
135 0.00125202\\
136 0.00125419\\
137 0.00125636\\
138 0.00125854\\
139 0.00126073\\
140 0.00126291\\
141 0.0012651\\
142 0.00126729\\
143 0.00126948\\
144 0.00127167\\
145 0.00127387\\
146 0.00127606\\
147 0.00127825\\
148 0.00128044\\
149 0.00128263\\
150 0.00128482\\
151 0.00128701\\
152 0.00128919\\
153 0.00129137\\
154 0.00129355\\
155 0.00129572\\
156 0.00129789\\
157 0.00130005\\
158 0.00130221\\
159 0.00130436\\
160 0.00130651\\
161 0.00130865\\
162 0.00131078\\
163 0.00131291\\
164 0.00131503\\
165 0.00131715\\
166 0.00131925\\
167 0.00132135\\
168 0.00132345\\
169 0.00132553\\
170 0.0013276\\
171 0.00132967\\
172 0.00133173\\
173 0.00133378\\
174 0.00133582\\
175 0.00133785\\
176 0.00133987\\
177 0.00134188\\
178 0.00134388\\
179 0.00134587\\
180 0.00134785\\
181 0.00134982\\
182 0.00135178\\
183 0.00135373\\
184 0.00135567\\
185 0.0013576\\
186 0.00135952\\
187 0.00136143\\
188 0.00136332\\
189 0.00136521\\
190 0.00136708\\
191 0.00136894\\
192 0.00137079\\
193 0.00137263\\
194 0.00137446\\
195 0.00137627\\
196 0.00137808\\
197 0.00137987\\
198 0.00138165\\
199 0.00138342\\
200 0.00138518\\
201 0.00138693\\
202 0.00138866\\
203 0.00139038\\
204 0.00139209\\
205 0.00139379\\
206 0.00139548\\
207 0.00139715\\
208 0.00139882\\
209 0.00140047\\
210 0.00140211\\
211 0.00140374\\
212 0.00140535\\
213 0.00140696\\
214 0.00140855\\
215 0.00141013\\
216 0.0014117\\
217 0.00141325\\
218 0.0014148\\
219 0.00141633\\
220 0.00141785\\
221 0.00141936\\
222 0.00142086\\
223 0.00142235\\
224 0.00142382\\
225 0.00142529\\
226 0.00142674\\
227 0.00142818\\
228 0.00142961\\
229 0.00143103\\
230 0.00143244\\
231 0.00143383\\
232 0.00143522\\
233 0.00143659\\
234 0.00143796\\
235 0.00143931\\
236 0.00144065\\
237 0.00144198\\
238 0.0014433\\
239 0.00144461\\
240 0.0014459\\
241 0.00144719\\
242 0.00144847\\
243 0.00144973\\
244 0.00145099\\
245 0.00145224\\
246 0.00145347\\
247 0.0014547\\
248 0.00145591\\
249 0.00145711\\
250 0.00145831\\
251 0.00145949\\
252 0.00146067\\
253 0.00146183\\
254 0.00146299\\
255 0.00146413\\
256 0.00146527\\
257 0.0014664\\
258 0.00146751\\
259 0.00146862\\
260 0.00146972\\
261 0.00147081\\
262 0.00147188\\
263 0.00147295\\
264 0.00147402\\
265 0.00147507\\
266 0.00147611\\
267 0.00147714\\
268 0.00147817\\
269 0.00147919\\
270 0.00148019\\
271 0.00148119\\
272 0.00148219\\
273 0.00148317\\
274 0.00148414\\
275 0.00148511\\
276 0.00148606\\
277 0.00148701\\
278 0.00148796\\
279 0.00148889\\
280 0.00148981\\
281 0.00149073\\
282 0.00149164\\
283 0.00149254\\
284 0.00149344\\
285 0.00149432\\
286 0.0014952\\
287 0.00149607\\
288 0.00149694\\
289 0.00149779\\
290 0.00149864\\
291 0.00149948\\
292 0.00150032\\
293 0.00150114\\
294 0.00150197\\
295 0.00150278\\
296 0.00150359\\
297 0.00150438\\
298 0.00150518\\
299 0.00150596\\
300 0.00150674\\
301 0.00150752\\
302 0.00150828\\
303 0.00150904\\
304 0.00150979\\
305 0.00151054\\
306 0.00151128\\
307 0.00151202\\
308 0.00151274\\
309 0.00151347\\
310 0.00151418\\
311 0.00151489\\
312 0.0015156\\
313 0.00151629\\
314 0.00151699\\
315 0.00151767\\
316 0.00151835\\
317 0.00151903\\
318 0.0015197\\
319 0.00152036\\
320 0.00152102\\
321 0.00152167\\
322 0.00152232\\
323 0.00152296\\
324 0.00152359\\
325 0.00152422\\
326 0.00152485\\
327 0.00152547\\
328 0.00152608\\
329 0.00152669\\
330 0.0015273\\
331 0.0015279\\
332 0.00152849\\
333 0.00152908\\
334 0.00152967\\
335 0.00153025\\
336 0.00153083\\
337 0.0015314\\
338 0.00153196\\
339 0.00153252\\
340 0.00153308\\
341 0.00153363\\
342 0.00153418\\
343 0.00153473\\
344 0.00153526\\
345 0.0015358\\
346 0.00153633\\
347 0.00153686\\
348 0.00153738\\
349 0.00153789\\
350 0.00153841\\
351 0.00153892\\
352 0.00153942\\
353 0.00153992\\
354 0.00154042\\
355 0.00154091\\
356 0.0015414\\
357 0.00154189\\
358 0.00154237\\
359 0.00154285\\
360 0.00154332\\
361 0.00154379\\
362 0.00154426\\
363 0.00154472\\
364 0.00154518\\
365 0.00154563\\
366 0.00154608\\
367 0.00154653\\
368 0.00154698\\
369 0.00154742\\
370 0.00154785\\
371 0.00154829\\
372 0.00154872\\
373 0.00154915\\
374 0.00154957\\
375 0.00154999\\
376 0.00155041\\
377 0.00155082\\
378 0.00155123\\
379 0.00155164\\
380 0.00155205\\
381 0.00155245\\
382 0.00155285\\
383 0.00155324\\
384 0.00155364\\
385 0.00155402\\
386 0.00155441\\
387 0.00155479\\
388 0.00155518\\
389 0.00155555\\
390 0.00155593\\
391 0.0015563\\
392 0.00155667\\
393 0.00155704\\
394 0.0015574\\
395 0.00155776\\
396 0.00155812\\
397 0.00155847\\
398 0.00155883\\
399 0.00155918\\
400 0.00155952\\
401 0.00155987\\
402 0.00156021\\
403 0.00156055\\
404 0.00156089\\
405 0.00156122\\
406 0.00156156\\
407 0.00156189\\
408 0.00156221\\
409 0.00156254\\
410 0.00156286\\
411 0.00156318\\
412 0.0015635\\
413 0.00156382\\
414 0.00156413\\
415 0.00156444\\
416 0.00156475\\
417 0.00156506\\
418 0.00156536\\
419 0.00156566\\
420 0.00156596\\
421 0.00156626\\
422 0.00156656\\
423 0.00156685\\
424 0.00156714\\
425 0.00156743\\
426 0.00156772\\
427 0.001568\\
428 0.00156829\\
429 0.00156857\\
430 0.00156885\\
431 0.00156913\\
432 0.0015694\\
433 0.00156967\\
434 0.00156995\\
435 0.00157022\\
436 0.00157048\\
437 0.00157075\\
438 0.00157101\\
439 0.00157127\\
440 0.00157154\\
441 0.00157179\\
442 0.00157205\\
443 0.00157231\\
444 0.00157256\\
445 0.00157281\\
446 0.00157306\\
447 0.00157331\\
448 0.00157355\\
449 0.0015738\\
450 0.00157404\\
451 0.00157428\\
452 0.00157452\\
453 0.00157476\\
454 0.001575\\
455 0.00157523\\
456 0.00157546\\
457 0.0015757\\
458 0.00157593\\
459 0.00157615\\
460 0.00157638\\
461 0.00157661\\
462 0.00157683\\
463 0.00157705\\
464 0.00157727\\
465 0.00157749\\
466 0.00157771\\
467 0.00157793\\
468 0.00157814\\
469 0.00157836\\
470 0.00157857\\
471 0.00157878\\
472 0.00157899\\
473 0.0015792\\
474 0.0015794\\
475 0.00157961\\
476 0.00157981\\
477 0.00158002\\
478 0.00158022\\
479 0.00158042\\
480 0.00158062\\
481 0.00158081\\
482 0.00158101\\
483 0.00158121\\
484 0.0015814\\
485 0.00158159\\
486 0.00158178\\
487 0.00158197\\
488 0.00158216\\
489 0.00158235\\
490 0.00158253\\
491 0.00158272\\
492 0.0015829\\
493 0.00158309\\
494 0.00158327\\
495 0.00158345\\
496 0.00158363\\
497 0.00158381\\
498 0.00158398\\
499 0.00158416\\
500 0.00158433\\
501 0.00158451\\
502 0.00158468\\
503 0.00158485\\
504 0.00158502\\
505 0.00158519\\
506 0.00158536\\
507 0.00158553\\
508 0.00158569\\
509 0.00158586\\
510 0.00158602\\
511 0.00158618\\
512 0.00158635\\
513 0.00158651\\
514 0.00158667\\
515 0.00158683\\
516 0.00158698\\
517 0.00158714\\
518 0.0015873\\
519 0.00158745\\
520 0.00158761\\
521 0.00158776\\
522 0.00158791\\
523 0.00158806\\
524 0.00158822\\
525 0.00158836\\
526 0.00158851\\
527 0.00158866\\
528 0.00158881\\
529 0.00158895\\
530 0.0015891\\
531 0.00158924\\
532 0.00158939\\
533 0.00158953\\
534 0.00158967\\
535 0.00158981\\
536 0.00158995\\
537 0.00159009\\
538 0.00159023\\
539 0.00159037\\
540 0.0015905\\
541 0.00159064\\
542 0.00159077\\
543 0.00159091\\
544 0.00159104\\
545 0.00159117\\
546 0.00159131\\
547 0.00159144\\
548 0.00159157\\
549 0.0015917\\
550 0.00159183\\
551 0.00159195\\
552 0.00159208\\
553 0.00159221\\
554 0.00159233\\
555 0.00159246\\
556 0.00159258\\
557 0.00159271\\
558 0.00159283\\
559 0.00159295\\
560 0.00159307\\
561 0.00159319\\
562 0.00159331\\
563 0.00159343\\
564 0.00159355\\
565 0.00159367\\
566 0.00159379\\
567 0.0015939\\
568 0.00159402\\
569 0.00159413\\
570 0.00159425\\
571 0.00159436\\
572 0.00159447\\
573 0.00159459\\
574 0.0015947\\
575 0.00159481\\
576 0.00159492\\
577 0.00159503\\
578 0.00159514\\
579 0.00159525\\
580 0.00159536\\
581 0.00159547\\
582 0.00159557\\
583 0.00159568\\
584 0.00159578\\
585 0.00159589\\
586 0.00159599\\
587 0.0015961\\
588 0.0015962\\
589 0.0015963\\
590 0.00159641\\
591 0.00159651\\
592 0.00159661\\
593 0.00159671\\
594 0.00159681\\
595 0.00159691\\
596 0.00159701\\
597 0.00159711\\
598 0.0015972\\
599 0.0015973\\
600 0.0015974\\
601 0.00159749\\
602 0.00159759\\
603 0.00159768\\
604 0.00159778\\
605 0.00159787\\
606 0.00159797\\
607 0.00159806\\
608 0.00159815\\
609 0.00159824\\
610 0.00159833\\
611 0.00159842\\
612 0.00159852\\
613 0.00159861\\
614 0.00159869\\
615 0.00159878\\
616 0.00159887\\
617 0.00159896\\
618 0.00159905\\
619 0.00159913\\
620 0.00159922\\
621 0.00159931\\
622 0.00159939\\
623 0.00159948\\
624 0.00159956\\
625 0.00159965\\
626 0.00159973\\
627 0.00159981\\
628 0.0015999\\
629 0.00159998\\
630 0.00160006\\
631 0.00160014\\
632 0.00160022\\
633 0.0016003\\
634 0.00160038\\
635 0.00160046\\
636 0.00160054\\
637 0.00160062\\
638 0.0016007\\
639 0.00160078\\
640 0.00160085\\
641 0.00160093\\
642 0.00160101\\
643 0.00160109\\
644 0.00160116\\
645 0.00160124\\
646 0.00160131\\
647 0.00160139\\
648 0.00160146\\
649 0.00160153\\
650 0.00160161\\
651 0.00160168\\
652 0.00160175\\
653 0.00160183\\
654 0.0016019\\
655 0.00160197\\
656 0.00160204\\
657 0.00160211\\
658 0.00160218\\
659 0.00160225\\
660 0.00160232\\
661 0.00160239\\
662 0.00160246\\
663 0.00160253\\
664 0.0016026\\
665 0.00160267\\
666 0.00160273\\
667 0.0016028\\
668 0.00160287\\
669 0.00160293\\
670 0.001603\\
671 0.00160307\\
672 0.00160313\\
673 0.0016032\\
674 0.00160326\\
675 0.00160332\\
676 0.00160339\\
677 0.00160345\\
678 0.00160352\\
679 0.00160358\\
680 0.00160364\\
681 0.0016037\\
682 0.00160377\\
683 0.00160383\\
684 0.00160389\\
685 0.00160395\\
686 0.00160401\\
687 0.00160407\\
688 0.00160413\\
689 0.00160419\\
690 0.00160425\\
691 0.00160431\\
692 0.00160437\\
693 0.00160443\\
694 0.00160449\\
695 0.00160454\\
696 0.0016046\\
697 0.00160466\\
698 0.00160472\\
699 0.00160477\\
700 0.00160483\\
701 0.00160489\\
702 0.00160494\\
703 0.001605\\
704 0.00160505\\
705 0.00160511\\
706 0.00160516\\
707 0.00160522\\
708 0.00160527\\
709 0.00160533\\
710 0.00160538\\
711 0.00160543\\
712 0.00160549\\
713 0.00160554\\
714 0.00160559\\
715 0.00160564\\
716 0.0016057\\
717 0.00160575\\
718 0.0016058\\
719 0.00160585\\
720 0.0016059\\
721 0.00160595\\
722 0.001606\\
723 0.00160605\\
724 0.0016061\\
725 0.00160615\\
726 0.0016062\\
727 0.00160625\\
728 0.0016063\\
729 0.00160635\\
730 0.0016064\\
731 0.00160645\\
732 0.00160649\\
733 0.00160654\\
734 0.00160659\\
735 0.00160664\\
736 0.00160668\\
737 0.00160673\\
738 0.00160678\\
739 0.00160682\\
740 0.00160687\\
741 0.00160692\\
742 0.00160696\\
743 0.00160701\\
744 0.00160705\\
745 0.0016071\\
746 0.00160714\\
747 0.00160719\\
748 0.00160723\\
749 0.00160727\\
750 0.00160732\\
751 0.00160736\\
752 0.00160741\\
753 0.00160745\\
754 0.00160749\\
755 0.00160753\\
756 0.00160758\\
757 0.00160762\\
758 0.00160766\\
759 0.0016077\\
760 0.00160774\\
761 0.00160779\\
762 0.00160783\\
763 0.00160787\\
764 0.00160791\\
765 0.00160795\\
766 0.00160799\\
767 0.00160803\\
768 0.00160807\\
769 0.00160811\\
770 0.00160815\\
771 0.00160819\\
772 0.00160823\\
773 0.00160827\\
774 0.00160831\\
775 0.00160835\\
776 0.00160838\\
777 0.00160842\\
778 0.00160846\\
779 0.0016085\\
780 0.00160854\\
781 0.00160857\\
782 0.00160861\\
783 0.00160865\\
784 0.00160869\\
785 0.00160872\\
786 0.00160876\\
787 0.0016088\\
788 0.00160883\\
789 0.00160887\\
790 0.0016089\\
791 0.00160894\\
792 0.00160897\\
793 0.00160901\\
794 0.00160905\\
795 0.00160908\\
796 0.00160912\\
797 0.00160915\\
798 0.00160918\\
799 0.00160922\\
800 0.00160925\\
801 0.00160929\\
802 0.00160932\\
803 0.00160935\\
804 0.00160939\\
805 0.00160942\\
806 0.00160945\\
807 0.00160949\\
808 0.00160952\\
809 0.00160955\\
810 0.00160959\\
811 0.00160962\\
812 0.00160965\\
813 0.00160968\\
814 0.00160971\\
815 0.00160975\\
816 0.00160978\\
817 0.00160981\\
818 0.00160984\\
819 0.00160987\\
820 0.0016099\\
821 0.00160993\\
822 0.00160996\\
823 0.00160999\\
824 0.00161003\\
825 0.00161006\\
826 0.00161009\\
827 0.00161012\\
828 0.00161015\\
829 0.00161017\\
830 0.0016102\\
831 0.00161023\\
832 0.00161026\\
833 0.00161029\\
834 0.00161032\\
835 0.00161035\\
836 0.00161038\\
837 0.00161041\\
838 0.00161044\\
839 0.00161046\\
840 0.00161049\\
841 0.00161052\\
842 0.00161055\\
843 0.00161058\\
844 0.0016106\\
845 0.00161063\\
846 0.00161066\\
847 0.00161068\\
848 0.00161071\\
849 0.00161074\\
850 0.00161077\\
851 0.00161079\\
852 0.00161082\\
853 0.00161084\\
854 0.00161087\\
855 0.0016109\\
856 0.00161092\\
857 0.00161095\\
858 0.00161097\\
859 0.001611\\
860 0.00161103\\
861 0.00161105\\
862 0.00161108\\
863 0.0016111\\
864 0.00161113\\
865 0.00161115\\
866 0.00161118\\
867 0.0016112\\
868 0.00161123\\
869 0.00161125\\
870 0.00161127\\
871 0.0016113\\
872 0.00161132\\
873 0.00161135\\
874 0.00161137\\
875 0.00161139\\
876 0.00161142\\
877 0.00161144\\
878 0.00161147\\
879 0.00161149\\
880 0.00161151\\
881 0.00161153\\
882 0.00161156\\
883 0.00161158\\
884 0.0016116\\
885 0.00161163\\
886 0.00161165\\
887 0.00161167\\
888 0.00161169\\
889 0.00161172\\
890 0.00161174\\
891 0.00161176\\
892 0.00161178\\
893 0.0016118\\
894 0.00161182\\
895 0.00161185\\
896 0.00161187\\
897 0.00161189\\
898 0.00161191\\
899 0.00161193\\
900 0.00161195\\
901 0.00161197\\
902 0.00161199\\
903 0.00161202\\
904 0.00161204\\
905 0.00161206\\
906 0.00161208\\
907 0.0016121\\
908 0.00161212\\
909 0.00161214\\
910 0.00161216\\
911 0.00161218\\
912 0.0016122\\
913 0.00161222\\
914 0.00161224\\
915 0.00161226\\
916 0.00161228\\
917 0.0016123\\
918 0.00161231\\
919 0.00161233\\
920 0.00161235\\
921 0.00161237\\
922 0.00161239\\
923 0.00161241\\
924 0.00161243\\
925 0.00161245\\
926 0.00161247\\
927 0.00161248\\
928 0.0016125\\
929 0.00161252\\
930 0.00161254\\
931 0.00161256\\
932 0.00161258\\
933 0.00161259\\
934 0.00161261\\
935 0.00161263\\
936 0.00161265\\
937 0.00161267\\
938 0.00161268\\
939 0.0016127\\
940 0.00161272\\
941 0.00161274\\
942 0.00161275\\
943 0.00161277\\
944 0.00161279\\
945 0.0016128\\
946 0.00161282\\
947 0.00161284\\
948 0.00161285\\
949 0.00161287\\
950 0.00161289\\
951 0.0016129\\
952 0.00161292\\
953 0.00161294\\
954 0.00161295\\
955 0.00161297\\
956 0.00161299\\
957 0.001613\\
958 0.00161302\\
959 0.00161303\\
960 0.00161305\\
961 0.00161307\\
962 0.00161308\\
963 0.0016131\\
964 0.00161311\\
965 0.00161313\\
966 0.00161314\\
967 0.00161316\\
968 0.00161317\\
969 0.00161319\\
970 0.0016132\\
971 0.00161322\\
972 0.00161323\\
973 0.00161325\\
974 0.00161326\\
975 0.00161328\\
976 0.00161329\\
977 0.00161331\\
978 0.00161332\\
979 0.00161334\\
980 0.00161335\\
981 0.00161337\\
982 0.00161338\\
983 0.00161339\\
984 0.00161341\\
985 0.00161342\\
986 0.00161344\\
987 0.00161345\\
988 0.00161346\\
989 0.00161348\\
990 0.00161349\\
991 0.00161351\\
992 0.00161352\\
993 0.00161353\\
994 0.00161355\\
995 0.00161356\\
996 0.00161357\\
997 0.00161359\\
998 0.0016136\\
999 0.00161361\\
1000 0.00161363\\
};
\addlegendentry{full}
